Edge-based Local Push for Personalized PageRank

Personalized PageRank (PPR) is a popular node proximity metric in graph mining and network research. Given a graph G=(V,E) and a source node $s \in V$, a single-source PPR (SSPPR) query asks for the PPR value $\vpi(u)$ with respect to s, which represents the relative importance of node u in the context of the source node s. Among existing algorithms for SSPPR queries, LocalPush is a fundamental method which serves as a cornerstone for subsequent algorithms. In LocalPush, a push operation is a crucial primitive operation, which distributes the probability at a node u to ALL u's neighbors via the corresponding edges. Although this push operation works well on unweighted graphs, unfortunately, it can be rather inefficient on weighted graphs. In particular, on unbalanced weighted graphs where only a few of these edges take the majority of the total weight among them, the push operation would have to distribute insignificant probabilities along those edges which just take the minor weights, resulting in expensive overhead. To resolve this issue, we propose the EdgePush algorithm, a novel method for computing SSPPR queries on weighted graphs. EdgePush decomposes the aforementioned push operations in edge-based push, allowing the algorithm to operate at the edge level granularity. Hence, it can flexibly distribute the probabilities according to edge weights. Furthermore, our EdgePush allows a fine-grained termination threshold for each individual edge, leading to a superior complexity over LocalPush. Notably, we prove that EdgePush improves the theoretical query cost of LocalPush by an order of up to O(n) when the graph's weights are unbalanced, both in terms of $\ell_1$-error and normalized additive error. Our experimental results demonstrate that EdgePush significantly outperforms state-of-the-art baselines in terms of query efficiency on large motif-based and real-world weighted graphs.

==> others.tex <==
%\section{Optimization with $l_1$ regularization} 
\section{Connection with Coordinate Descent} 
\label{sec:others}

%\subsection{Connection with coordinate descent in APPR} 
%Review the differences between power method and local push algorithm. Power method treats the PPR vector $\vpi$ as a unit, and update it by executing the matrix-vector multiplication $\P \vpi $ in each iteration. While local push approach separates the multiplication $\P \vpi $ into pieces. In each push step, it picks one coordinate of vector $\vpi$ to update its neighbors' PPR values. Hence, local push algorithm is actually a coordinate solver of the linear equation~\eqref{eqn:PPR-def}. Power method can be viewed as the aggregations of multiple steps of local push operations. 
%Even though after adequate push operations, the local push 
%method can finally achieve the same results as that of power method, the discrete push operation provides better scalability and 
%After adequate push operations and multiplication iterations, the two methods can finally achieve the same PPR results. 

%Furthermore, \cite{fountoulakis2019variational} points out that the local push method for APPR is equivalent to a coordinate descent process with the following objective function:   
%\begin{equation}\label{eqn:obj-variational}
%f(\epi)=\frac{1}{2} \epi^\top \mathbf{Q}\epi-\alpha \s^\top \D^{-\frac{1}{2}}\epi, 
%\end{equation}
%where $\mathbf{Q}=\D^{-\frac{1}{2}}\cdot \left[\D-\frac{1-\alpha}{2}(\D+\A)\right]\cdot \D^{-\frac{1}{2}}$, and $\epi=\D^{-\frac{1}{2}}\vpi$. 
%It classifies the problem to solve the PPR linear system~\eqref{eqn:PPR-def} as an optimization process to seek the minimum value of the above objective function. Actually, this objective function is not unique to solve the PPR problem. By converting to a more generalized version, we can unify this formula as the optimization function commonly used in multiple graph learning tasks, such as graph signal processing~\cite{Survey-graphSignalIII}, graph neural networks~\cite{zhang2020revisiting-GCNoptfunc}, feature/label propagation~\cite{zhou2003learning-LP-optfunc, huang2020C&S}, and so on. 
%\begin{lemma}
%The objective function shown in equation~\eqref{eqn:obj-variational} can be generalized as the following formula:  
%\begin{equation}\label{eqn:obj-PPR}
% f(\epi)=\frac{1-\alpha}{2}\cdot \left(\epi^\top \mathbf{L}\epi\right)+\frac{\alpha}{2} %\left\|\epi-\bm{s}\right\|_2^2, 
%\end{equation}
%where $\L$ is the laplacian matrix that $\L=\I-\D^{-\frac{1}{2}}\A \D^{-\frac{1}{2}}$. 
%\end{lemma}
%When $\P=\A \D^{-1}$ in local clustering tasks, we need to set $\s=\D^{-\frac{1}{2}}\cdot \frac{\D \cdot \bm{1}}{2m}$, where $\bm{1}\in \mathcal{R}^n$ denotes the vector each entry of which is 1. The real initial vector in clustering tasks $\frac{\D \cdot \bm{1}}{2m}$ represents to choose the seed node according to the degrees. Then the optimal $\epi^*$ that minimizes this objective function satisfies $\epi^*=\D^{-\frac{1}{2}}\vpi$. While in most graph learning tasks, the transition probability matrix $\P$ in equation~\eqref{eqn:PPR-def} is always set as $\Dn \A \Dn$. Then we have $\epi^*=\vpi$. And $\s$ can be the feature vector, node label, or graph signal vector depending on specific applications. 

%\begin{proof}
%We can first rewrite the expression of matrix $\mathbf{Q}$ as $\mathbf{Q}=\frac{1+\alpha}{2}\I-\frac{1-\alpha}{2}\D^{-\frac{1}{2}}\A \D^{-\frac{1}{2}}$. Let $\beta=\frac{2\alpha}{1+\alpha}$ and substitute $\alpha$ with $\beta$ in equation~\eqref{eqn:obj-variational}. Then we can derive that 
%\begin{equation}\label{eqn:fq1}
%    f(\epi)=\frac{\epi^\top \left(\I-(1-\beta)\D^{-\frac{1}{2}}\A \D^{-\frac{1}{2}} \right)\epi}{2(2-\beta)}-\frac{\beta\s^\top \D^{-\frac{1}{2}}\epi}{2-\beta}.
%\end{equation} 
%Note that our goal is to find the optimal $\epi^*$ that minimizes the objective function. Hence, $\epi^*$ satisfies $\nabla f(\epi^*)=0$, where $\nabla f$ represents the gradient of the function $f$. Scale up $f(\epi)$ by constant factors will not influence the solutions of $\nabla f(\epi^*)=0$. So equation~\eqref{eqn:fq1} can be further converted to the following function by multiplying $(2-\beta)$.  
%\begin{equation} \label{eqn:fq2}
%\begin{aligned}
%    &f(\epi)
%    =\frac{1}{2}\epi^\top \left(\I-(1-\beta)\D^{-\frac{1}{2}}\A \D^{-\frac{1}{2}} \right)\epi-\beta\cdot \s^\top \D^{-\frac{1}{2}}\epi\\
%    &=\frac{1-\beta}{2}\epi^\top \left(\I-\D^{-\frac{1}{2}}\A \D^{-\frac{1}{2}} \right)\epi+\frac{\beta}{2}\cdot \left\| \epi-\D^{-\frac{1}{2}}\s\right\|_2^2.
%\end{aligned}
%\end{equation}
%In the last equation, we add $\left( \s^\top \D^{-1} \s \right)$ to $f(\epi)$ because the constant term $\left( \s^\top \D^{-1} \s \right)$ is excluded from the gradient of $f(\epi)$. Note that the objective function presented in ~\cite{fountoulakis2019variational} focuses on local clustering tasks, where $\P=\A \D^{-1}$ in the definition equation~\eqref{eqn:PPR-def}. While in most graph learning tasks, $\P$ is always extended to  $\P=\D^{-\frac{1}{2}}\A \D^{-\frac{1}{2}}$ that $\vpi=(1-\alpha)\D^{-\frac{1}{2}}\A \D^{-\frac{1}{2}} \vpi+\alpha \s$. To generalized the objective function, we find that
%\begin{equation}\nonumber
%    \begin{aligned}
%\vpi
%&=\sum_{i=0}^\infty (1-\alpha)^i \left(\Dn \A \Dn \right)^i\s\\
%&=\Dn \cdot \sum_{i=0}^\infty (1-\alpha)^i \left(\A \D^{-1} \right)^i \Dp \s. 
%    \end{aligned}
%\end{equation}
%By substituting $\s'=\Dp \s$, and multiplying $\Dn$ with $\vpi'=\sum_{i=0}^\infty (1-\alpha)^i \left(\A \D^{-1} \right)^i \s'$, we can unify the push process under the two settings of $\P$. Hence, the objective function shown in equation~\eqref{eqn:fq2} can be further generalized as 
%\begin{equation}\nonumber
%\begin{aligned}
%    f(\epi)=\frac{1-\beta}{2}\epi^\top \left(\I-\D^{-\frac{1}{2}}\A \D^{-\frac{1}{2}} \right)\epi+\frac{\beta}{2}\cdot \left\|\epi-\s\right\|_2^2, 
%\end{aligned}
%\end{equation}
%which follows the Lemma. 
%\end{proof}

%We can understand this objective function from two aspects: the first term $\epi^\top \L \epi$ tries to impose some smoothness on the propagation vector, that the related vertices on the graph tend to show similar propagation results. While the second term $\left\|\epi-\s \right\|_2^2$ uses $\ell_2$ regularization to keep $\epi$ not far away from the initial vector $\s$. To minimize the objective function $f(\epi)$, the coordinate descent algorithm proposed in ~\cite{fountoulakis2019variational} updates each coordinate of $\epi$ via: 
%$\epi=\epi-\nabla_i f(\epi) \cdot e_i$, where $\nabla_i f (\epi)$ is the $i_{th}$ entry of vector $\nabla f(\epi)$. Note that 
%\begin{equation} \nonumber
%    \nabla f(\epi)=(1-\alpha)\mathbf{L}\epi+\alpha(\epi -\s)=\left(\I-(1-\alpha)\P \right)\epi-\alpha \s, 
%\end{equation}
%which exactly equals to the changes of $\epi$ by the iterative equation $\epi=(1-\alpha)\P\epi+\alpha \s$ given in PPR's definition. Benchmarking the residue and reserve vector $\r$ and $\epi$, the work~\cite{fountoulakis2019variational} states that actually $\vpi=\Dp \epi$ and 
%$\nabla f(\epi)=-\alpha \Dn \r$. The same as the push step shown in Algorithm~\ref{alg:push-APPR}, the coordinate descent step updates $\epi(i)$ and all entries $j$ of $\nabla f(\epi)$ that $v_j \in N_i$.  


\begin{algorithm}[t]
    \caption{Coordinate descent solver for $\min f(q)$ \label{alg:coordinate-APPR}}
    \begin{algorithmic}
    \STATE {\bfseries Input:} Graph $G=(V,E)$, initial vector $\s$, teleport probability $\alpha$, threshold $r_{max}$
    \STATE {\bfseries Output:} the estimation of PPR vector $\vpi$
    \end{algorithmic}
\begin{algorithmic}[1]
    \STATE {$\epi \gets \bm{0}$, and thus $\nabla f(\epi)\gets -\alpha \Dn \s$};
    \WHILE{$\left\|\frac{1}{\alpha}\Dn \nabla f(\epi)\right\|_\infty \ge r_{max}$}
        \STATE {pick an arbitrary $i$ such that $\frac{1}{\alpha \sqrt{d_i}} \nabla_i f(\epi) \le -r_{max}$};
        \STATE {$\epi(i)\gets\epi(i)-\nabla_i f(\epi)$};
        \FOR{every neighbors $v_j\in N_i$}
            \STATE {$\nabla_j f(\epi)\gets \nabla_i f(\epi)-\frac{1-\alpha}{\sqrt{d_i}\sqrt{d_j}}\nabla_i f(\epi)$};
        \ENDFOR
        \STATE {$\nabla_i f(\epi) \gets 0 $};
    \ENDWHILE
\STATE {\bfseries return}  $\vpi=\Dp \epi$
\end{algorithmic}
\end{algorithm}



Algorithm~\ref{alg:coordinate-APPR} is the pseudo code of the whole coordinate descent process given in ~\cite{fountoulakis2019variational}. Note that in every step, it still needs to touch every neighbor to update the gradient (Line 5-7). One step of coordinate descent can still have the risk to cost $O(n)$ on some dense graphs. Actually, we can prove that under the vanilla push framework, we must scan the neighbors and update their residues simultaneously in one push step to guarantee accuracy (proof shown in Section~\ref{sec:analysis}). Even though the coordinate descent solver provides us a variational perspective to understand PPR computation, stuck in the vanilla push structure may limits more elaborate analysis for efficiency improvement. Hence, there emerges some interesting questions that: is it possible to break through the structure of node-based push, and update the residue only for one adjacent edge instead of all adjacent nodes? Can we correspondingly design a more flexible coordinate descent approach to support the edge-based push and cast more precise analysis on push efficiency?




\begin{equation}\nonumber
 f(\bm{\pi})=\frac{1-\alpha}{2}\cdot \left(\bm{\pi}^\top \mathbf{L}\bm{\pi}\right)+\frac{\alpha}{2} \left\|\bm{\pi}-\bm{s}\right\|_2^2+\alpha \cdot r_{max} \left\|\mathbf{D}\Pi \right\|_1. 
\end{equation}


\subsection{Connection to LASSO regression}
\begin{equation}\nonumber
\min_{\bm{x}\in \mathcal{R}^n}\frac{1}{2} \left\|\mathbf{A}\bm{x}-\bm{b}\right\|_2^2, \quad \text{subject to} \left\|\bm{x}\right\|_1\le \mu.    
\end{equation}


\begin{equation}\nonumber
    \min_{\bm{x}\in \mathcal{R}^n}\frac{1}{2} \left\|\mathbf{A}\bm{x}-\bm{b}\right\|_2^2+\lambda \left\|\bm{x}\right\|_1. 
\end{equation}


% \subsection{Related work}

% \paragraph{Global propagation. } APPNP
% \paragraph{Local propagation. } PPRGo, GBP


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> reponse.tex <==
\clearpage
\setcounter{page}{1}
\section*{author response} \label{sec:response}
We thank the reviewers for the insightful and constructive comments. Following the suggestions, we revise our paper and the major changes are highlighted in {\hz blue}. Our responses to the major concerns of reviewers are as follows. 

\subsection*{Reviewer 1} \label{sec:r1}
\review{\bf D1}: {\em In the time complexity analysis part above Fact 3, named ``Cost per edge-based push", the authors said that each $A_{uv}$ and the priorities $k_{u}(v)$ can be represented by $O(\log n)$ bits, so all the values can be mapped to an integer domain with size bounded by $O(poly(n))$. It seems to me that $\alpha$ will also affect the values of $Q_{uv}$ (then affect the values of priorities of $k_{u}(v)$). So, does $\alpha$ also need such a constraint? Please explain.}

\header{\bf Response: }

\review{\bf D2}: {\em Following D1, when sorting the edge weights and priorities by Radix sort, if the Radix sort is performed from the least significant bit (or most significant bit), does it still need $O(\log n)$ passes over the weights and priorities? (If yes, the time complexity becomes $O(\log n m)$?) Or can the authors explain how Radix sort is performed here?}

\header{\bf Response: }

\review{\bf D3}: {\em Following D2, if the time complexity becomes larger, does this change affect the overall time complexity analysis in Section 5.1, and comparison to the localpush algorithm in Section 5.3?}

\header{\bf Response: }


\review{\bf D4}: {\em For the trends shown in Figure 7 and 8, what will happen if more points are provided with smaller error values? Please try to provide more results for those two algorithms with smaller values. Will PowforPush outperform EdgePush in other datasets (except YT)? If this is the case, can some explanation be provided?}

\header{\bf Response: } Thanks for pointing out this. We revise Figure~\ref{fig:l1error-query-real_l1} and Figure~\ref{fig:maxerror-query-real_l1} with more points for smaller $\ell_1$-error. 



\subsection*{Reviewer 2} \label{sec:r2}
\review{\bf D1}: {\em Minor note: the legend of Figure 2 has an incomplete second sentence}

\header{\bf Response: }
Corrected as advised. Thanks for pointing out this! 


%\review{\bf D2}: {\em My major concern regards the applicability of the method:}

\review{\bf D2.1}: {\em In Section 1, I found the "toy example" discussion informative and technically convincing. However, empirical evidence for such extreme skew in edge weights should also be provided.}

\header{\bf Response: } Thanks for the advice. Graphs with heavily unbalanced edge weights are commonly used in multiple applications, such as label propagation, spectral clustering and image segmentation. We add detailed description in the Introduction section (Section~\ref{sec:intro}). 

%For example, in the case of label propagation, the input is a set of multi-dimensional data points $X=\{x_1,x_2,...,x_n\} \in \mathbb{R}^m$. Each data point indicates a word, a paragraph, an image pixel, or other entity depending on the downstream task. Only a small percentage of data points are labeled with the remainder are unlabeled. The goal of label propagation is to predict the labels of the unlabeled data points based on the consistency assumption: nearby points or points on the same structure are likely to have the same label. Such a problem is called semi-supervised and a typical pipeline is to construct a fully-connected affinity graph first, then to apply semi-supervised learning method on the affinity graphs. In particular, Zhou et al.~\cite{zhou2004consistency} propose to utilize the PPR values computed on the affinity graph as the probabilities to predict unknown labels. 

%Considering the full-connected affinity graph, the nodes corresponds to the data points and the weight of edge connecting points $x_i$ and $x_j$ is defined as follows: 
%\begin{align*}
%    \A_{ij}=\exp\left(-\|x_i-x_j\|^2/2\sigma^2\right), 
%\end{align*}
%where $\|x_i-x_j\|$ denotes the distance (e.g., the Euclidean distance) between points $x_i$ and $x_j$. Note that the distance $\|x_i-x_j\|$ is exponential to the edge weight $\A_{ij}$. Thus, small differences among pairwise distances can lead to significantly-skewed edge weights distribution. Consequently, to apply \localpush for PPR computation on such heavily unbalanced weighted graphs can invoke expensive but unnecessary time cost. 



\vspace{+2mm}
\review{\bf D2.2}: {\em In Section 6, one would expect real-world graphs with real-world edge weights. Without this, it is unclear if we are studying a real problem. The synthetic motif-based method for creating edge weights for unweighted graphs is not completely satisfying. What about other methods for creating weights? Why this method? How do these compare to the structure of real weights in real-world graphs?}

\header{\bf Response: } Thanks for pointing out this. We add the experiments on four real-world datasets with real edge weights (i.e. TA, TH, BC, SP). Please refer to Section~\ref{sec:exp} for details. 

\vspace{+2mm}
\review{\bf D2.3}: {\em In Section 6, one would also expect a sensitivity study with synthetic graphs, to find the border between graph structures which are beneficial for EdgePush and not particularly beneficial, relative to the baselines. For example, a study of the impact of (a, b)-unbalancedness, for changing values of (a,b). Are the situations which are beneficial to EdgePush common?}

\header{\bf Response: } Thanks for the advice. We evaluate the sensitivity of \edgepush to the weight unbalancedness in Figure~\ref{fig:maxerror-query-add-sensitivity} and Figure~\ref{fig:l1error-query-sensitivity}. Please refer to Section~\ref{subsec:sensitivity} for details. 



 


\subsection*{Reviewer 3} \label{sec:r3}
\review{\bf W1}: {\em A minor concern is that the weighted graphs used in the experiment are generated from unweighted graphs. The empirical results would be more convincing to see results on real-world weighted graphs.}

\header{\bf Response: } Thanks for the suggestion. We add the experiments on four real-world weighted graphs (i.e. TA, TH, BC and SP). Please see Section~\ref{sec:exp} for details. 


\review{\bf W2}: {\em The experiment compares EdgePush against FORA, which is a hybrid of LocalPush and random walk. Since the submission claims that EdgePush is a superior substitute for LocalPush, it will be interesting to explore if EdgePush can be paired with random walk to improve overall performance as well as efficiency.}

\header{\bf Response: } We add the experiments to combine EdgePush with Monte-Carlo based random walks in Figure {\hz TODO}. Please see Section {\hz TODO} for details. 




==> responseFull.tex <==
\clearpage
\setcounter{page}{1}
\setcounter{figure}{0} 
\renewcommand\thefigure{R.\arabic{figure}}
\setcounter{table}{0}
\renewcommand\thetable{R.\arabic{table}}
\setcounter{equation}{0}
\section*{author response} \label{sec:response}
%We thank the reviewers for the insightful and constructive comments. Following the suggestions, we revise our paper and the major changes are highlighted in {\hz blue}. Our responses to the major concerns of reviewers are as follows. 
We thank the reviewers for their insightful and constructive comments. Based on the reviewers' suggestions, the major changes we made in the revised paper can be summarized as three aspects: 
\begin{itemize}
\vspace{-1mm}
    \item {\bf Theoretical Analyses: } (for Reviewer 1) 
    
    We explicitly introduced the word RAM theoretical model and provided further explanations on the time complexity analysis of \edgepush. Relevant revisions are mainly in Section~\ref{sec:pre} and ~\ref{sec:algorithm}. 
    
    \item {\bf Applicability Illustrations: } (for Reviewer 2)  
    
    We provided a commonly used graph type, the affinity graph, as the example where weighted graphs have severely unbalanced edge weights. Relevant revisions are mainly in Section~\ref{sec:intro}. Notably, even on the graphs without severely unbalanced weight distributions, \edgepush can still significantly outperform the state-of-the-art methods from the empirical aspect. 
    
    \item {\bf Supplementary Experiments: } (for Reviewers 1, 2 and 3) 
    
    We revised the experiments on motif-based weighted graphs. And we added experiments on four real-world graphs with real edge weights. The experimental results demonstrate the effectiveness and superiority of \edgepush over all the state-of-the-art competitors. Additionally, we included a sensitivity test to evaluate the impact of the unbalancedness on the performance of \edgepush. %Finally, we combined \edgepush with Monte-Carlo based random walks as an interesting attempt for future studies. 
    Relevant revisions are mainly in Section~\ref{sec:exp}. 
    %\item In Introduction (Section~\ref{sec:intro}), we introduce affinity graphs, which are weighted graphs with heavily unbalanced edge weight and are commonly used in a wide range of applications (Details can be found in the revised paper). The importance of affinity graphs demonstrates the applicability of weighted graphs whose edges are unbalanced. 
    %\item In Preliminaries (Section~\ref{sec:pre}) and the Algorithm section (Section~\ref{sec:algorithm}), we explicitly introduce the word RAM model and provide further explanations in the time complexity analysis for \edgepush. 
    %\item In Experiments (Section~\ref{sec:exp}), we add experiments on four new real-world graphs with real edge weights. 
    %The experimental results demonstrate the effectiveness and superiority of \edgepush over all the state-of-the-art competitors.
    %Extensive experiments demonstrate the applicability and  effectiveness of \edgepush. 
    %\item Additionally, in Experiments (Section~\ref{sec:exp}), a sensitivity test is added for evaluation on the impact of the unbalancedness on the performance of \edgepush. The experimental results concur with our analysis that \edgepush are in favor of the case that the edge weights are unbalanced.
    %unbalanced weighted graphs. 
    %Moreover, we also show that \edgepush performs no worse than that of \localpush on balanced graphs. 
\end{itemize}

In the revised paper, the major changes were highlighted in {\hz blue}. Our responses to the major concerns of reviewers were as follows. For the sake of readability, we also presented the supplementary tables and figures in the response letter, with captions beginning with R.1. 


\subsection*{Reviewer 1} \label{sec:r1}
\review{\bf D1}: {\em In the time complexity analysis part above Fact 3, named ``Cost per edge-based push", the authors said that each $A_{uv}$ and the priorities $k_{u}(v)$ can be represented by $O(\log n)$ bits, so all the values can be mapped to an integer domain with size bounded by $O(poly(n))$. It seems to me that $\alpha$ will also affect the values of $Q_{uv}$ (then affect the values of priorities of $k_{u}(v)$). So, does $\alpha$ also need such a constraint? Please explain.}

\header{\bf Response: } Thanks for pointing out this. The expression ``each $A_{uv}$ and the priorities $k_{u}(v)$ can be represented by $O(\log n)$ bits" was originally intended to indicate that we derived the analysis under the word RAM model. Following the advice, in the revised paper, we explicitly introduced the word RAM model in the Preliminaries section (Section~\ref{sec:pre}).  

Specifically, the word RAM model (word random-access machine) is first proposed by Fredman et al.~\cite{fredman1993surpassing} to simulate the actual executions of programs implemented by well-adopted programming languages, e.g., C and C++, in real-world computers. The word RAM model assumes a random-access machine can do bitwise operations on a single word of $w$ bits. The value of $w$ is related to the problem size. More specifically, let $n$ denote the problem size; the word RAM model assumes $w = \Theta \left( \log n \right)$. 
In other words, in the word RAM model, the memory is divided into words, each of $w$ bits; and each word can represent integers in the range from $0$ to $2^w -1$. 
%Additionally, the word RAM model assumes the word size matches the problem size. That is, for size-$n$ inputs, the word RAM model assumes $w=\Theta\left(\log n\right)$. 
Thus, in the word RAM model, basic operations on words such as arithmetic, comparison and logical shifts can be performed in constant time.

In this paper, we analyzed all of the theoretical complexities under the word RAM model. 
Following the aforementioned convention of the model,
%Following the assumption of word RAM model, in our paper, 
we assumed that every numerical value, such as the edge weight $\A_{uv}$ and the constant teleport probability $\alpha$ in PPR computation, can fit into $O(1)$ words of $O(w)$ bits.
As the problem size studied in this paper is upper bounded by the input graph size $O(n + m) \subseteq O(n^2)$, every numerical value can be thus represented by $O(\log n)$ bits.
%With some abuse of notation, we still use $n$ to denote the problem size following the convention of theoretical computer science. Thus, equivalently, we assume $\alpha$ and each $\A_{uv}$ can be represented by $O(\log n)$ bits. 
We noted that this assumption is mild and realistic, simply because most (if not all) real-world computers can only support computations on floating-point numbers up to limited precision. %That said, these floating-point numbers are not true real values.
%do compute with floating point numbers (instead of exact real numbers with infinite precision) which can be represented by discrete bits. 

%The word RAM model (word random-access machine) is first proposed by Fredman et al.~\cite{fredman1993surpassing} to simulate programming languages like C. It assumes a random-access machine can do bitwise operations on a single word of $w$ bits. In other words, in the word RAM model, the memory is divided into words of length $w$ bits and each word can store integers up to size $2^w$. Additionally, the word RAM model assumes the word size matches the problem size. That is, for size-$n$ inputs, the word RAM model assumes $w=\Theta\left(\log n\right)$. Thus, under the word RAM model, basic operations such as arithmetic, comparison and logical shifts can be done in constant time. 

%Following the assumption of word RAM model, in our paper, we assume all the numerical values can be fit into $O(1)$ words, including each edge weight $\A_{uv}$ and the constant teleport probability $\alpha$ in PPR computation. With some abuse of notation, we still use $n$ to denote the problem size following the convention of theoretical computer science. Thus, equivalently, we assume $\alpha$ and each $\A_{uv}$ can be represented by $O(\log n)$ bits. Note that this assumption is mild because most actual computers do compute with floating point numbers (instead of exact real numbers with infinite precision) which can be represented by discrete bits. 

\begin{comment}
\begin{figure*}[t]
    \begin{minipage}[t]{1\textwidth}
		\centering
		\vspace{-5mm}
		%    \begin{footnotesize}
		\begin{tabular}{cccc}
			%\multicolumn{4}{c}{\hspace{-4mm} \includegraphics[height=5mm]{./Figs/legend_large.eps}} \vspace{-1mm} \\
			\hspace{-4mm} \includegraphics[width=43mm]{./Figs/l1err-query-YT_l1.eps} &
			%\hspace{-3mm} \includegraphics[height=25mm]{./Figs/HKPR-maxerr-query-DB.eps} &
    		\hspace{-3mm} \includegraphics[width=43mm]{./Figs/l1err-query-LJ_l1.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/l1err-query-IC_l1.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/l1err-query-OL_l1.eps} 
		\end{tabular}
		\vspace{-5mm}
		\caption{{\em $\ell_1$-error} v.s. query time on motif-based weighted graphs.}
		\label{fig:l1error-query-real_l1-response}
		\vspace{-1mm}
    \end{minipage}
    
	\begin{minipage}[t]{1\textwidth}
		\centering
		\vspace{+1mm}
		%    \begin{footnotesize}
		\begin{tabular}{cccc}
			%\multicolumn{4}{c}{\hspace{-4mm} \includegraphics[height=5mm]{./Figs/legend_large.eps}} \vspace{-1mm} \\
			\hspace{-4mm} \includegraphics[width=43mm]{./Figs/maxerr-query-YT_l1.eps} &
			%\hspace{-3mm} \includegraphics[height=25mm]{./Figs/HKPR-maxerr-query-DB.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/maxerr-query-LJ_l1.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/maxerr-query-IC_l1.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/maxerr-query-OL_l1.eps} 
		\end{tabular}
		\vspace{-5mm}
		\caption{{\em MaxAddErr} v.s. query time on motif-based weighted graphs.}
		\label{fig:maxerror-query-real_l1-response}
		\vspace{-1mm}
    \end{minipage}



    \begin{minipage}[t]{1\textwidth}
		\centering
		\vspace{+1mm}
		%    \begin{footnotesize}
		\begin{tabular}{cccc}
			%\multicolumn{4}{c}{\hspace{-4mm} \includegraphics[height=5mm]{./Figs/legend_large.eps}} \vspace{-1mm} \\
			\hspace{-4mm} \includegraphics[width=43mm]{./Figs/precision-query-YT_l1.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/precision-query-LJ_l1.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/precision-query-IC_l1.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/precision-query-OL_l1.eps} 
		\end{tabular}
		\vspace{-4mm}
		\caption{{\em precision@50} v.s. query time on motif-based weighted graphs.}
		\label{fig:precision-query-real_l1-response}
		\vspace{-4mm}
	\end{minipage}
\end{figure*}
\end{comment}

\begin{figure*}[t]
	\begin{minipage}[t]{1\textwidth}
		\centering
		\vspace{-5mm}
		%    \begin{footnotesize}
		\begin{tabular}{cccc}
			%\multicolumn{4}{c}{\hspace{-4mm} \includegraphics[height=5mm]{./Figs/legend_large.eps}} \vspace{-1mm} \\
			\hspace{-4mm} \includegraphics[width=43mm]{./Figs/maxerr-query-TA_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/maxerr-query-TH_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/maxerr-query-BC_AddErr.eps}&
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/maxerr-query-SP_AddErr.eps}\\
			%\hspace{-3mm} \includegraphics[width=37mm]{./Figs/maxerr-query-BT_AddErr.eps}\\ 
		\end{tabular}
		\vspace{-5mm}
		\caption{{\em normalized MaxAddErr} v.s. query time on real weighted graphs.}
		\label{fig:maxerror-query-real_pro-real-response}
		\vspace{-1mm}
    \end{minipage}

    \begin{minipage}[t]{1\textwidth}
		\centering
		\vspace{+1mm}
		%    \begin{footnotesize}
		\begin{tabular}{cccc}
			%\multicolumn{4}{c}{\hspace{-4mm} \includegraphics[height=5mm]{./Figs/legend_large.eps}} \vspace{-1mm} \\
			\hspace{-4mm} \includegraphics[width=43mm]{./Figs/precision-query-TA_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/precision-query-TH_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/precision-query-BC_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/precision-query-SP_AddErr.eps}\\
			%\hspace{-4mm} \includegraphics[width=37mm]{./Figs/precision-query-BT_AddErr.eps}\\
		\end{tabular}
		\vspace{-4mm}
		\caption{{\em normalized precision@50} v.s. query time on real weighted graphs.}
		\label{fig:precision-query-real_pro-real-response}
		\vspace{-1mm}
	\end{minipage}


	\begin{minipage}[t]{1\textwidth}
		\centering
		\vspace{+1mm}
		%    \begin{footnotesize}
		\begin{tabular}{cccc}
			%\multicolumn{4}{c}{\hspace{-4mm} \includegraphics[height=5mm]{./Figs/legend_large.eps}} \vspace{-1mm} \\
			\hspace{-4mm} \includegraphics[width=43mm]{./Figs/conductance-query-TA_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/conductance-query-TH_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/conductance-query-BC_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/conductance-query-SP_AddErr.eps} \\
			%\hspace{-4mm} \includegraphics[width=37mm]{./Figs/conductance-query-BT_AddErr.eps}\\
		\end{tabular}
		\vspace{-4mm}
		\caption{{\em conductance} v.s. query time on real weighted graphs.}
		\label{fig:conductance-query-real_pro-real-response}
		\vspace{-2mm}
	\end{minipage}
\end{figure*}


\review{\bf D2}: {\em Following D1, when sorting the edge weights and priorities by Radix sort, if the Radix sort is performed from the least significant bit (or most significant bit), does it still need $O(\log n)$ passes over the weights and priorities? (If yes, the time complexity becomes $O(\log n m)$?) Or can the authors explain how Radix sort is performed here?}

\header{\bf Response: } 
%Sorry for the confusion. 
Following our response to D1, we assume the word RAM model where
%in this paper, we analyze all of the theoretical complexities under the word RAM model. And we assume every the numerical value, such as the edge weight $\A_{uv}$ and the constant teleport probability $\alpha$ in PPR computation, can fit into $O(1)$ words of $O(w)$ bits. By the assumption, we can verify that all values of 
each edge weight value $\A_{uv}$ and each priority value $k_u(v)$ can be represented by $O(\log n)$ bits. In this model, we can sort %, and hence, each of them can be mapped to an integer domain with size bounded by
%can be mapped to an integer domain with size bounded by 
%$O(\text{poly}(n))$. 
all the edge weights $\A_{uv}$ and all the priorities $k_u(v)$ in $O(m)$ time with the standard Radix sort~\cite{knuth1998art}. The key idea is to perform Counting Sort on every $\log n$ bits rather than on every bit, which reduces the number of passes from $O(\log n)$ to $O(1)$.
%More precisely, the Radix Sort under the word RAM Model conducts sorting {\em word}-wise, rather than {\em bit}-wise. During the sorting process, it sorts all the elements first by the {\em least significant word} (i.e., the least significant $O(\log n)$ bits), then by the {\em second-least significant word} (i.e., the next $O(\log n)$ bits) and so on so forth, up to the {\em most significant word}. As a result, the Radix Sort requires only $O\left( \frac{\log{\text{poly}(n)}}{\log n}\right)=O(1)$ rounds; and each round takes $O(m)$ time. The overall $O(m)$ running time of Radix Sort thus follows.
%More precisely, there are $O(m)$ elements (i.e. all the edge weights $\A_{uv}$ and all the priorities $k_u(v)$) to be sorted using the Radix Sort. Under the word RAM model, the Radix Sort conducts {\em Counting Sort} for every $\log n$ bits of the $O(m)$ elements, rather than for each bit. 
Specifically, during the sorting process, the Radix Sort first performs Counting Sort on the least significant $\log n$ bits, then by the next $\log n$ bits and so on so forth, up to the most significant $\log n$ bits. As a result, the Radix Sort requires only $O\left( \frac{\log{\text{poly}(n)}}{\log n}\right)=O(1)$ passes of Counting Sort. By ~\cite{cormen2009introduction}, the time cost of Counting Sort can be bounded by $O(m+n)=O(m)$ to sort $O(m)$ elements in the range from $0$ to $2^{\log n}-1=n-1$. Thus, the overall running time of Radix Sort is bounded by $O(m)$, which follows the proof. 
%In each pass, the Radix Sort performs Counting Sort on the $O(m)$ elements with $\log n$ bits per element. By~\cite{cormen2009introduction}, such Counting Sort costs $O(m+n)=O(m)$ time.
%In each round of Counting Sort, there are $O(m)$ elements, each of which is in the numerical range from $0$ to $2^{\log n}-1=n-1$.  Recall that the Radix Sort conducts $O(1)$ rounds of Counting Sort. The overall $O(m)$ running time of Radix Sort thus follows. 
%As a result, to sort $O(m)$ elements with $O(\log n)$ bits, the Radix Sort process requires only $O\left( \frac{\log{\text{poly}(n)}}{\log n}\right)=O(1)$ rounds of counting sort. 
%to sort $O(m)$ with size bounded by $k$ using the counting sort, the time complexity can be bounded by $O(m+k)$. Corresponding, the overall running time of Radix Sort can be bounded by $O(m+2^{\log n})=O(m+n)=O(m)$.

%By the assumption, it can be verified that all values of edge weights $\A_{uv}$ and the priorities $k_u(v)$ can be mapped to an integer domain with size bounded by $O(\text{poly}(n))$. Therefore, by the standard Radix sort~\cite{knuth1998art}, all the edge weights $\A_{uv}$ and all the priorities $k_u(v)$ can be sorted in $O(m)$ time. More precisely, the Radix Sort under the word RAM Model conducts sorting {\em word}-wise, rather than {\em bit}-wise. During the sorting process, we sort all the elements first by the {\em least significant word}, then by the {\em second-least significant word}, etc., up to the {\em most significant word}. Therefore, the Radix Sort process costs $O\left(m\cdot \frac{\log{\text{poly}(n)}}{\log n}\right)=O(m)$ time. 

%Thanks for pointing out this. In Section~\ref{subsec:candidate} of the revised paper, we add the detailed descriptions on the process of Radix Sort under the word RAM model. 

\review{\bf D3}: {\em Following D2, if the time complexity becomes larger, does this change affect the overall time complexity analysis in Section 5.1, and comparison to the localpush algorithm in Section 5.3?}

\header{\bf Response: } By the discussion in the above response to D1 and D2, the overall time complexity analysis shown in the analysis part (Section~\ref{sec:analysis}) holds under the word RAM model. 
%On the other hand, if we focus on exact real numbers with infinite precision, instead of floating point numbers used by most actual computers, the analysis can be transferred to the real RAM model~\cite{shamos1978realRAM}. In the case of real RAM model, 


\review{\bf D4}: {\em For the trends shown in Figure 7 and 8, what will happen if more points are provided with smaller error values? Please try to provide more results for those two algorithms with smaller values. Will PowforPush outperform EdgePush in other datasets (except YT)? If this is the case, can some explanation be provided?}

\header{\bf Response: } Thanks for pointing out this. We revised  Figure~\ref{fig:l1error-query-real_l1} and Figure~\ref{fig:maxerror-query-real_l1} with more points for smaller $\ell_1$-error. %(as shown in Figure~\ref{fig:l1error-query-real_l1-response} and ~\ref{fig:maxerror-query-real_l1-response}). 
Please refer to Section~\ref{subsec:l1} for details. 
We observed that \edgepush outperforms the competitors in terms of query efficiency on all datasets with large $\ell_1$-error. With the decreasing of $\ell_1$-error, the plot curves of the three methods gradually overlap. 
%This is because with strict $\ell_1$-error constraints, \edgepush and PowForPush both have to touch most of edges in the graph, which have actually become powermethod. 
This is because with strict $\ell_1$-error constraints, \edgepush has to touch most of edges in the graph, which have actually become PowForPush. 
%This is because with strict $\ell_1$-error constraints, \edgepush and PowForPush both have to touch most of edges in the graph, leading to the cost of $O(m)$. 

On the other hand, recall that the $\ell_1$-error is defined as the sum of additive error over all nodes in the graph (i.e. $\sum_{u\in V}|\epi(u)-\vpi(u)|$). Hence, even with some relatively large $\ell_1$-error, the (normalized) additive error can be small enough for real applications (e.g., local clustering~\cite{FOCS06_FS}).    



%This is due to the switching technique applied to PowForPush and \edgepush. Specifically, as we mentioned in Section~\ref{sec:related} and Section~\ref{subsec:l1}, PowForPush is the state-of-the-art algorithm for high-precision SSPPR queries, which gradually switches \localpush to Power Method with decreasing $\ell_1$-error. More precisely, in the first phase, PowForPush adopts \localpush to compute the SSPPR queries. When the current number of {\em active} nodes is greater than a specified {\em scanThreshold}, PowForPush switches to Power Method by performing a sequential scan technique to access active nodes for the \lpush operation. A node is called active if its residue is larger than the global termination threshold $\theta$. The rationale behind this switching mechanism is that sequential scan is often more efficient if the number of random access is relatively large.

%Inspired by PowForPush, in our experiments, we apply the same switching technique to our \edgepush for the fairness of comparison. Specifically, when the number of edges in the candidate set $\mathcal{C}$ is significant compared to the graph size, we switch \edgepush to Power Method by performing sequential scanning to access active edges and stop maintaining the two-level structure for each node. An edge $\la u,v \ra\in \bar{E}$ is active if its edge residue is larger than the termination threshold $\theta(u,v)$. With strict $\ell_1$-error constraints, the number of active nodes and edges in PowForPush and \edgepush are both greater than the {\em scanThreshold}. Hence, the two methods both switch to Power Method for high-precision SSPPR queries. Therefore, the three methods (i.e. \edgepush, PowForPush and powermethod) show similar performance with strict $\ell_1$-error constraints. Notably, \edgepush and PowForPush continue to outperform powermethod on IC and OL by a small margin, owing mostly to the optimization tricks (i.e. sequential scanning and dynamic $\ell_1$-error threshold) adopted in \edgepush and PowForPush after switching. 


\begin{figure*}[t]
	\begin{minipage}[t]{1\textwidth}
		\centering
		\vspace{-5mm}
		%    \begin{footnotesize}
		\begin{tabular}{cccc}
			%\multicolumn{4}{c}{\hspace{-4mm} \includegraphics[height=5mm]{./Figs/legend_large.eps}} \vspace{-1mm} \\
			\hspace{-6mm}
			\includegraphics[width=43mm]{./Figs/maxerr-query-AG01_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/maxerr-query-AG1_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/maxerr-query-AG13_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/maxerr-query-AG20_AddErr.eps} \\
			\hspace{-2mm} (a) {\small $\left(\sum_{v\in V}n_v\hspace{-0.5mm}\cdot \hspace{-0.5mm} \cos^2\p_v\right)/m=0.01$}  &
			\hspace{0mm} (b) {\small $\left(\sum_{v\in V}n_v\hspace{-0.5mm}\cdot \hspace{-0.5mm} \cos^2\p_v\right)/m=0.14$} &
			\hspace{0mm} (c) {\small $\left(\sum_{v\in V}n_v\hspace{-0.5mm}\cdot \hspace{-0.5mm} \cos^2\p_v\right)/m=0.41$} &
			\hspace{0mm} (d) {\small $\left(\sum_{v\in V}n_v\hspace{-0.5mm}\cdot \hspace{-0.5mm} \cos^2\p_v\right)/m=0.7$} \\
			%\hspace{-4mm} \includegraphics[width=37mm]{./Figs/maxerr-query-BT_l1.eps}\\
		\end{tabular}
		\vspace{-3mm}
		\caption{{\em normalized MaxAddErr} v.s. query time for unbalancedness analysis}
		\label{fig:maxerror-query-add-sensitivity-response}
		\vspace{-1mm}
    \end{minipage}
    
    \begin{minipage}[t]{1\textwidth}
		\centering
		\vspace{+1mm}
		%    \begin{footnotesize}
		\begin{tabular}{cccc}
			%\multicolumn{4}{c}{\hspace{-4mm} \includegraphics[height=5mm]{./Figs/legend_large.eps}} \vspace{-1mm} \\
			\hspace{-4mm} \includegraphics[width=43mm]{./Figs/l1err-query-AG01_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/l1err-query-AG1_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/l1err-query-AG13_AddErr.eps} &
			\hspace{-3mm} \includegraphics[width=43mm]{./Figs/l1err-query-AG20_AddErr.eps} \\
			\hspace{+2mm} (a) { $\cos^2\p=0.01$}  &
			\hspace{+2mm} (b) { $\cos^2\p=0.14$} &
			\hspace{+2mm} (c) { $\cos^2\p=0.38$} &
			\hspace{+2mm} (d) { $\cos^2\p=0.66$} \\
			%\hspace{-4mm} \includegraphics[width=37mm]{./Figs/maxerr-query-BT_l1.eps}\\
		\end{tabular}
		\vspace{-3mm}
		\caption{{\em $\ell_1$-error} v.s. query time for unbalancedness analysis}
		\label{fig:l1error-query-sensitivity-response}
		%\vspace{-1mm}
    \end{minipage}
\end{figure*}


\vspace{-2mm}
\subsection*{Reviewer 2} \label{sec:r2}
\vspace{-1mm}
\review{\bf D1}: {\em Minor note: the legend of Figure 2 has an incomplete second sentence}

\header{\bf Response: }
Corrected as advised. Thanks for pointing out this! 



%\review{\bf D2}: {\em My major concern regards the applicability of the method:}

\review{\bf D2.1}: {\em In Section 1, I found the "toy example" discussion informative and technically convincing. However, empirical evidence for such extreme skew in edge weights should also be provided.}

\header{\bf Response: } 
Thanks for pointing out this. Our response can be summarized into the following four points: 
\vspace{-1mm}
\begin{itemize}
    \item Figure~\ref{fig:weighted_graph} is just an extremely bad case for \localpush. From the theoretical aspect, we used Figure~\ref{fig:weighted_graph} to show that \edgepush can outperform \localpush by up to a $O(n)$ factor on such severely unbalanced graphs (e.g. on a complete graph each node of which shares the same structure as node $u$ in Figure~\ref{fig:weighted_graph}, proved in Lemma~\ref{lem:cos-l1} and Lemma~\ref{lem:cos-add}). However, we argue that, on the graphs with less unbalanced edge weights, \edgepush can still outperform \localpush in terms of theoretical cost bound. In fact, the expected time complexity of \edgepush is never worse than that of \localpush even on unweighted graphs. %It's just when the edge weights are unbalanced, \edgepush achieves superior query efficiency over \localpush. 
    And the superiority of \edgepush over \localpush can be quantified by the unbalancedness of the weighted graphs (using $\cos^2 \p$ and $\left(\sum_{v\in V}n_v\hspace{-0.5mm}\cdot \hspace{-0.5mm} \cos^2\p_v\right)/m$ shown in Lemma~\ref{lem:cos-l1} and Lemma~\ref{lem:cos-add}). 
    \item From the empirical aspect, \edgepush can significantly outperform the state-of-the-art methods on the graphs without significantly unbalanced edge weight distributions. For example, in the revised paper, we added four real-world weighted graphs with real edge weights (the meta data is listed in Table~\ref{tbl:datasets-response} using bolded text). We showed that \edgepush consistently outperforms baseline methods in terms of query efficiency on the four real weighted graphs (shown in from Figure~\ref{fig:maxerror-query-real_pro-real-response}, Figure~\ref{fig:precision-query-real_pro-real-response} and Figure~\ref{fig:conductance-query-real_pro-real-response}). In particular, even on Threads (TH) whose $\cos^2 \p=0.97$, \edgepush still outperforms all baselines in terms of query efficiency, which demonstrates the effectiveness of \edgepush.
    \item In the Introduction of the revised paper, we provided an example of the weighted graphs with severely unbalanced edge weights: the affinity graphs. Affinity graphs are frequently used in a variety of applications~\cite{zhou2004consistency, ng2002spectral,ye2020affinity,zhu2014constructing,wang2020affinity,yang2019learning,yadav2021cross,yang2019relationship}. 
    %such as label propagation~\cite{zhou2004consistency}, spectral clustering~\cite{ng2002spectral,ye2020affinit} and image segmentation~\cite{zhu2014constructing,wang2020affinity,yang2019learning}. 
    The nodes in affinity graphs (denoted as data points $x_i\in \mathbb{R}^m$) represent entities in the given data source. Edges are fully connected and weighted, indicating the affinities between pairwise entities. %Affinity graphs are fully-connected weighted graphs where 
    More precisely, in affinity graphs, the weight of each edge connecting any nodes $x_i$ and $x_j$ is defined as: $\A_{ij}=\exp\left(-\|x_i-x_j\|^2/2\sigma^2\right)$. Here $\|x_i-x_j\|$ represents the distance (e.g., the Euclidean distance) between nodes $x_i$ and $x_j$. Note that the value of distance $\|x_i-x_j\|^2$ is exponential to the edge weight $\A_{ij}$. Thus, small differences among pairwise distances can lead to significantly-skewed edge weights distribution. On the other hand, computing PPR values on affinity graphs is a commonly adopted technique for label propagation~\cite{zhou2004consistency}, spectral clustering~\cite{ye2020affinity}, image segmentation~\cite{yang2019learning} and relationship profiling~\cite{yang2019relationship}. Consequently, to apply \localpush for PPR computation on such heavily unbalanced weighted graphs can invoke expensive but unnecessary time cost. This also illustrates the applicability of \edgepush. 
    \item In Table~\ref{tbl:datasets-response}, we list the $\cos^2 \p$ value of each graph used in our experiments (i.e. four motif-based weighted graphs showing in the first four lines, and four real weighted graphs shown in the last four lines). Recall that in Lemma~\ref{lem:cos-l1}, we introduce the $\cos^2 \p$ notation to evaluate the unbalancedness of the weighted graphs. And the smaller $\cos^2 \p$ is, the more unbalanced the weighted graph is. From Table~\ref{tbl:datasets-response}, we note that except Threads (TH), the other datasets have relatively small $\cos^2 \p$, indicating unbalanced edge weight distribution in real-world scenarios. 
    %we list the $\cos^2 \p$ value of each graph used in our experiments in Table~\ref{tbl:datasets-response} (Recall that we introduce the $\cos^2 \p$ notation to evaluate the unbalancedness of the weighted graphs. The smaller $\cos^2 \p$ is, the more unbalanced the weighted graph is, defined in Lemma~\ref{lem:cos-l1} and Lemma~\ref{lem:cos-add}). We note that even on Threads (TH) whose $\cos^2 \p=0.97$, \edgepush still outperforms all baselines in terms of query efficiency. This demonstrates the effectiveness of \edgepush. In other words, even on the weighted graphs without severely unbalanced edge weight distributions, \edgepush still performs clear improvements over the baseline methods. 
    %The expected time complexity of \edgepush is never worse than that of \localpush, even on unweighted graphs (proved in Lemma~\ref{lem:cos-l1} and Lemma~\ref{lem:cos-add}). In particular, when the edge weights are unbalanced, \edgepush achieves superior query efficiency over \localpush in terms of the trade-offs between the expected overall running time and the approximation error. 
    %\item In the paper, we prove that the superiority of \edgepush can be quantified by the unbalancedness of the weighted graphs (shown in Table~\ref{tbl:intro-compare}). And we introduce the $\cos^2 \p$ notation to evaluate the unbalancedness of the weighted graphs (the smaller $\cos^2 \p$, the more unbalanced the weighted graph, defined in Lemma~\ref{lem:cos-l1} and Lemma~\ref{lem:cos-add}). We list the $\cos^2 \p$ value of each graph used in our experiments in Table~\ref{tbl:datasets-response}. We note that even on Threads (TH) whose $\cos^2 \p=0.97$, \edgepush still outperforms all baselines in terms of query efficiency. This demonstrates the effectiveness of \edgepush. In other words, even on the weighted graphs without severely unbalanced edge weight distributions, \edgepush still performs clear improvements over the baseline methods. 
    %\item In Table~\ref{tbl:datasets-response}, we list four motif-based weighted graphs (in the first four lines) and four real-world weighted graphs with real edge weights. We observe that except Threads (TH), the other datasets have relatively unbalanced edge weight distribution with small $\cos^2 \p$. Furthermore, from Figure~\ref{fig:maxerror-query-real_pro-real-response}, Figure~\ref{fig:precision-query-real_pro-real-response} and Figure~\ref{fig:conductance-query-real_pro-real-response}, we notice that \edgepush significantly outperforms state-of-the-art baselines in terms of query efficiency on real-world weighted graphs. This also demonstrates the applicability of \edgepush from the empirical aspect. 
\end{itemize}



%Thanks for the advice. Graphs with severely unbalanced edge weights are frequently used in a variety of applications, such as label propagation~\cite{zhou2004consistency}, spectral clustering~\cite{ng2002spectral} and image segmentation~\cite{zhu2014constructing,wang2020affinity,yang2019learning}. In Section~\ref{sec:intro}, we add more illustrations for the applications to employ the weighted graphs with significantly unbalanced edge weights. 

%For example, in the case of label propagation, the input is a set of multi-dimensional data points $X=\{x_1,x_2,...,x_n\} \in \mathbb{R}^m$. Each data point indicates a word, a paragraph, an image pixel, or other entity depending on the downstream task. Only a small percentage of data points are labeled with the remainder are unlabeled. The goal of label propagation is to predict the labels of the unlabeled data points based on the consistency assumption: nearby points or points on the same structure are likely to have the same label. Such a problem is called semi-supervised and a typical pipeline is to construct a fully-connected affinity graph first, then to apply semi-supervised learning method on the affinity graphs. In particular, Zhou et al.~\cite{zhou2004consistency} propose to utilize the PPR values computed on the affinity graph as the probabilities to predict unknown labels. 

%Considering the full-connected affinity graph, the nodes corresponds to the data points and the weight of edge connecting points $x_i$ and $x_j$ is defined as $\A_{ij}=\exp\left(-\|x_i-x_j\|^2/2\sigma^2\right)$, where $\sigma^2$ is the variance of data points, and $\|x_i-x_j\|$ denotes the distance (e.g., the Euclidean distance) between points $x_i$ and $x_j$. Note that the distance $\|x_i-x_j\|$ is exponential to the edge weight $\A_{ij}$. Thus, small differences among pairwise distances can lead to significantly-skewed edge weights distribution. Consequently, to apply \localpush for PPR computation on such heavily unbalanced weighted graphs can invoke expensive but unnecessary time cost. 

%Additionally, in the experimental part, we add four real-world graphs with real edge weights: Tags (TA)~\cite{benson2018simplicial}, Threads (TH)~\cite{benson2018simplicial}, BlockChair (BC)~\cite{blockchair} and Spotify (SP)~\cite{kumar2020retrieving}. The meta data of these datasets are listed in the following table, where the columns named ``mean" and ``max" report the average and maximum edge weights of each graph. Note that except in TH, there are significant gaps between the mean and max edge weights in the other three datasets, which also demonstrates that the graphs with severely unbalanced edge weights are common in real world applications. 
\begin{table}[t]
	%\vspace{-2mm}
	\centering
	%\tblcapup
	\caption{Real-World Datasets.}
	\vspace{-4mm}
	%\tblcapdown
	\begin{small}
		%\begin{tabular}{|@{\hspace{+0.3mm}}l@{\hspace{+0.3mm}}|@{\hspace{+0.3mm}}r@{\hspace{+0.3mm}}|@{\hspace{+0.3mm}}r@{\hspace{+0.3mm}}|r|r|r@{\hspace{+0.3mm}}|@{\hspace{+0.3mm}}r@{\hspace{+0.3mm}}|} %p{1.3in}|}
		\begin{tabular}{|@{\hspace{+0.3mm}}l@{\hspace{+0.3mm}}|@{\hspace{+0.3mm}}r@{\hspace{+0.3mm}}|@{\hspace{+0.3mm}}r@{\hspace{+0.3mm}}|r|r|r@{\hspace{+0.3mm}}|} %p{1.3in}|}
		%\begin{tabular}{|@{\hspace{+2mm}}l@{\hspace{+2mm}}|@{\hspace{+2mm}}r@{\hspace{+2mm}}|@{\hspace{+2mm}}r@{\hspace{+2mm}}|r@{\hspace{+2mm}}|@{\hspace{+2mm}}r@{\hspace{+2mm}}|} %p{1.3in}|}
		%\begin{tabular}{|l|r|r|r|r|}
			\hline
			%{\bf Dataset} &  {\bf $\boldsymbol{\|\A\|_1}$} & {\bf $\boldsymbol{n}$} & {\bf $\boldsymbol{m}$}	 \\ \hline
			%\multirow{2}{*}{{\bf Dataset}}& \multirow{2}{*}{{\bf $\boldsymbol{n}$}} & \multirow{2}{*}{{\bf $\boldsymbol{m}$}} & \multicolumn{2}{c|}{{\bf Edge weight}} & \multirow{2}{*}{{\bf $\boldsymbol{{\cos}^2 \p}$}} & \multirow{2}{*}{{\bf $\boldsymbol{{\cos}^2\p_v}$}}	\\ \cline{4-5}
			\multirow{2}{*}{{\bf Dataset}}& \multirow{2}{*}{{\bf $\boldsymbol{n}$}} & \multirow{2}{*}{{\bf $\boldsymbol{m}$}} & \multicolumn{2}{c|}{{\bf Edge weight}} & \multirow{2}{*}{{\bf $\boldsymbol{{\cos}^2 \p}$}} \\ \cline{4-5}
			%\multirow{2}{*}{{\bf Dataset}}& \multirow{2}{*}{{\bf $\boldsymbol{n}$}} & \multirow{2}{*}{{\bf $\boldsymbol{m}$}} & \multicolumn{2}{c|}{{\bf Edge Weight}}	\\ \cline{4-5}
			%~ & & & {\bf mean} & {\bf max} & & \\ \hline
			~ & & & {\bf mean} & {\bf max} & \\ \hline
			%YouTube (YT) &  1,138,499 & 2,795,228 & 6.6 & 4,034 & 0.65 & 0.83 \\
			YouTube (YT) &  1,138,499 & 2,795,228 & 6.6 & 4,034 & 0.65\\
			%YouTube (YT) &  1,138,499 & 2,795,228 & 6.6 & 4,034 \\
			%DBLP-Author  & undirected & 5,425,963 & 17,298,032 \\
			% {Com-LiveJournal(CL)} & undirected & 3,997,962	& 34,681,189 \\
			%LiveJournal (LJ) & 1,714,381,584 & 4,847,571 & 68,475,391\\
			%LiveJournal (LJ) & 4,847,571 & 71,062,058 &24 & 4,445 & 0.51 & 0.89 \\
			LiveJournal (LJ) & 4,847,571 & 71,062,058 &24 & 4,445 & 0.51 \\
			%LiveJournal (LJ) & 4,847,571 & 71,062,058 &24 & 4,445 \\
		    %IndoChina (IC)	& 360,693,368,232 & 	7,414,768  &	191,606,827		\\
		    %IndoChina (IC)& 7,414,768  &295,191,370	& 1,221 & 178,448 & 0.31 & 0.89\\
		    IndoChina (IC)& 7,414,768  &295,191,370	& 1,221 & 178,448 & 0.31\\
		    %IndoChina (IC)& 7,414,768  &295,191,370	& 1,221 & 178,448 \\
			%Orkut-Links (OL) & 3,765,464,226 & 3,072,441 & 234,369,798 \\	
			%Orkut-Links (OL) & 3,072,441 & 202,392,682 & 18 & 9,145 & 0.69 & 0.85\\
			Orkut-Links (OL) & 3,072,441 & 202,392,682 & 18 & 9,145 & 0.69\\
			%Tags (TA) & 49,945 & 8,294,604 & 13 & 469,258 & 0.27 & 0.47\\ 
			{\bf Tags (TA)} & {\bf 49,945} & {\bf 8,294,604} & {\bf 13} & {\bf 469,258} & {\bf 0.27}\\ 
			%{\hz Threads (TH)} & {\hz 2,321,767} & {\hz 42,012,344} & {\hz 1.1} & {\hz 546} & {\hz 0.97} & {\hz 0.98}\\ 
			%Threads (TH) & 2,321,767 & 42,012,344 & 1.1 & 546 & 0.97 & 0.98\\ 
			{\bf Threads (TH)} & {\bf 2,321,767} & {\bf 42,012,344} & {\bf 1.1} & {\bf 546} & {\bf 0.97} \\ 
			%{\hz blockchair (BC)} & {\hz 595,753} & {\hz 1,773,544} &  {\hz 5.2} & {\hz 17,165} & {\hz 0.5} & {\hz 0.89} \\ 
			%BlockChair (BC) & 595,753 & 1,773,544 &  5.2 & 17,165 & 0.5 & 0.89\\ 
			{\bf BlockChair (BC)} & {\bf 595,753} & {\bf 1,773,544} & {\bf 5.2} & {\bf 17,165} & {\bf 0.5}\\ 
			%{\hz Spotify (SP)} & {\hz 3,604,308} & {\hz 3,854,964,026} & {\hz 8.6} & {\hz 2878K} & {\hz 0.29} & {\hz 0.53}\\ 
			%Spotify (SP) & 3,604,308 & 3,854,964,026 & 8.6 & 2,878,970 & 0.29 & 0.53\\
			{\bf Spotify (SP)} & {\bf 3,604,308} & {\bf 3,854,964,026} & {\bf 8.6} & {\bf 2,878,970} & {\bf 0.29} \\ 
			\hline
		\end{tabular}
	\end{small}
	\label{tbl:datasets-response}
	%\tbldown
	\vspace{-4mm}
\end{table}
 

%For example, in the case of label propagation, the input is a set of multi-dimensional data points $X=\{x_1,x_2,...,x_n\} \in \mathbb{R}^m$. Each data point indicates a word, a paragraph, an image pixel, or other entity depending on the downstream task. Only a small percentage of data points are labeled with the remainder are unlabeled. The goal of label propagation is to predict the labels of the unlabeled data points based on the consistency assumption: nearby points or points on the same structure are likely to have the same label. Such a problem is called semi-supervised and a typical pipeline is to construct a fully-connected affinity graph first, then to apply semi-supervised learning method on the affinity graphs. In particular, Zhou et al.~\cite{zhou2004consistency} propose to utilize the PPR values computed on the affinity graph as the probabilities to predict unknown labels. 

%Considering the full-connected affinity graph, the nodes corresponds to the data points and the weight of edge connecting points $x_i$ and $x_j$ is defined as follows: 
%\begin{align*}
%    \A_{ij}=\exp\left(-\|x_i-x_j\|^2/2\sigma^2\right), 
%\end{align*}
%where $\|x_i-x_j\|$ denotes the distance (e.g., the Euclidean distance) between points $x_i$ and $x_j$. Note that the distance $\|x_i-x_j\|$ is exponential to the edge weight $\A_{ij}$. Thus, small differences among pairwise distances can lead to significantly-skewed edge weights distribution. Consequently, to apply \localpush for PPR computation on such heavily unbalanced weighted graphs can invoke expensive but unnecessary time cost. 



\vspace{+2mm}
\review{\bf D2.2}: {\em In Section 6, one would expect real-world graphs with real-world edge weights. Without this, it is unclear if we are studying a real problem. The synthetic motif-based method for creating edge weights for unweighted graphs is not completely satisfying. What about other methods for creating weights? Why this method? How do these compare to the structure of real weights in real-world graphs?}

\header{\bf Response: } Thanks for the advice. We added the experiments on four real-world datasets with real edge weights (i.e. TA, TH, BC, SP). Specifically, Tags (TA) and Threads (TH) were derived from Stack Overflow, a well-known Q\&A (Question-and-Answer) website for programmers. In Tags (TA), nodes are tags of questions and edge weights are the number of questions jointly annotated by two tags. On the other hand, nodes in Threads (TH) represent users and the edge weight indicates how frequently two users appear in the same question thread. BlockChair (BC) is a bitcoin transaction network, where nodes are addresses and edge weights are the number of transactions between two addresses. In our experiments, we used the transactions records on December 5, 2021. Spotify (SP) is a music streaming network. The nodes in Spotify represent songs and the edge weight is the number of times that two songs appear in one session. More detailed descriptions of these real weighted datasets can be founded at~\cite{kumar2020retrieving}. 

In Figure~\ref{fig:maxerror-query-real_pro-real-response}, Figure~\ref{fig:precision-query-real_pro-real-response} and Figure~\ref{fig:conductance-query-real_pro-real-response}, we drew the trade-off plots between the query time and the normalized maximum additive error (denoted as \nadd), {\em normalized precision@50} and {\em conductance}, respectively. Please refer to Section~\ref{sec:exp} for detailed parameter settings. We observed that under the same \nadd, \npre or conductance, \edgepush takes the smallest query time among all these methods on all datasets. Notably, we found that the performance of all the methods on real weighted graphs are analogous to those on motif-based graphs, which shows the rational to use motif-based weighted graphs. Additionally, we observed that compared to the performance of \edgepush on TH, the superiorities of \edgepush over \localpush are more clear on TA, BC and SP. This concurs with our analysis that the superiority of \edgepush changes with the unbalancedness of edge weights.


\vspace{+2mm}
\review{\bf D2.3}: {\em In Section 6, one would also expect a sensitivity study with synthetic graphs, to find the border between graph structures which are beneficial for EdgePush and not particularly beneficial, relative to the baselines. For example, a study of the impact of (a, b)-unbalancedness, for changing values of (a,b). Are the situations which are beneficial to EdgePush common?}

\header{\bf Response: } Thanks for the advice. We evaluated the sensitivity of \edgepush to the weight unbalancedness in Figure~\ref{fig:maxerror-query-add-sensitivity-response} and ~\ref{fig:l1error-query-sensitivity-response}. Specifically, we generated four fully-connected affinity graphs whose $\cos^2 \p$ vary in $(0.01,0.14,0.38, 0.66)$, and $\left(\sum_{v\in V}n_v\hspace{-0.5mm}\cdot \hspace{-0.5mm} \cos^2\p_v\right)/m$ vary in $(0.01, 0.14, 0.41, 0.77)$. Please refer to 
the Technical Report~\cite{TechnicalReport}  for the detailed experimental settings. Recall that in Lemma~\ref{lem:cos-l1} and Lemma~\ref{lem:cos-add}, we introduced $\cos^2 \p$ and $\left(\sum_{v\in V}n_v\hspace{-0.5mm}\cdot \hspace{-0.5mm} \cos^2\p_v\right)/m$ to quantify the superiority of \edgepush over \localpush with $\ell_1$-error and normalized additive error. That is, the smaller $\cos^2 \p$ or $\left(\sum_{v\in V}n_v\hspace{-0.5mm}\cdot \hspace{-0.5mm} \cos^2\p_v\right)/m$ is, the more unbalanced the graph is. Accordingly, as seen in Figure~\ref{fig:maxerror-query-add-sensitivity-response} and Figure~\ref{fig:l1error-query-sensitivity-response}, we observed that the gaps between the trade-off lines of \edgepush and \localpush reduce from left to right, which is consistent with our analysis. 

Note that in our paper, we introduced two types of notions, $(a,b)$-unbalanced nodes (in Section~\ref{sec:intro}) and $\cos^2 \p$ (in Section~\ref{subsec:individual}), to evaluate the unbalancedness of the weighted graph. The notion of $(a,b)$-unbalanced nodes is more intuitive, while the $\cos^2 \p$ is more general and less restrictive (A detailed comparison between $(a,b)$-unbalanced and $\cos^2 \p$ is deferred to our Technical Report~\cite{TechnicalReport}). As a result, we adopted the notion of $\cos^2 \p$ to quantify the unbalancedness of weighted graphs in the sensitivity studies. 


\subsection*{Reviewer 3} \label{sec:r3}
\review{\bf W1}: {\em A minor concern is that the weighted graphs used in the experiment are generated from unweighted graphs. The empirical results would be more convincing to see results on real-world weighted graphs.}

\header{\bf Response: } Thanks for the advice. We added the experiments on four real-world weighted graphs (i.e. TA, TH, BC and SP). The meta data of the four real-world weighted graphs is listed in Table~\ref{tbl:datasets-response}. And the experimental results are presented in Figure~\ref{fig:maxerror-query-real_pro-real-response}, ~\ref{fig:precision-query-real_pro-real-response} and ~\ref{fig:conductance-query-real_pro-real-response}. Please see our responses to the D2.2 point of Reviewer 2 or Section~\ref{sec:exp} for detailed descriptions. 


\review{\bf W2}: {\em The experiment compares EdgePush against FORA, which is a hybrid of LocalPush and random walk. Since the submission claims that EdgePush is a superior substitute for LocalPush, it would be interesting to explore if EdgePush can be paired with random walk to improve overall performance as well as efficiency.}

\header{\bf Response: } %We added the experiments to combine EdgePush with Monte-Carlo based random walks in Figure {\hz TODO}. Please see Section {\hz TODO} for details. 
Thanks for the suggestion. Note that in our experiments, \edgepush has outperformed FORA and SpeedPPR in terms of query efficiency. How to further combine \edgepush with random walks to improve the overall performance is a non-trivial problem, which is beyond the scope of this paper. We leave this interesting problem as our future work. 



